Finding Robust Solutions to Stable Marriage

We study the notion of robustness in stable matching problems. We first define robustness by introducing (a,b)-supermatches. An $(a,b)$-supermatch is a stable matching in which if $a$ pairs break up it is possible to find another stable matching by changing the partners of those $a$ pairs and at most $b$ other pairs. In this context, we define the most robust stable matching as a $(1,b)$-supermatch where b is minimum. We show that checking whether a given stable matching is a $(1,b)$-supermatch can be done in polynomial time. Next, we use this procedure to design a constraint programming model, a local search approach, and a genetic algorithm to find the most robust stable matching. Our empirical evaluation on large instances show that local search outperforms the other approaches.

==> cactus_large_opt.tex <==
\cactus{Optimality ratio}{GA, LS}{b={mark=diamond*,blue!50,draw=blue!50!black}, c={mark=triangle*,yellow!50,draw=yellow!50!black}}{{{(0.0, 0.0) [b] },{(0.0, 0.0) [c] }}}


==> cactus_small_opt.tex <==
\cactus{Optimality ratio}{CP, GA, LS}{a={mark=*,red!50,draw=red!50!black}, b={mark=diamond*,blue!50,draw=blue!50!black}, c={mark=triangle*,yellow!50,draw=yellow!50!black}}{{{(0.0, 0.0) [a] (0.0005, 28.7) [a] (0.001, 30.8) [a] (0.0015, 31.3) [a] (0.002, 31.5) [a] (0.0025, 31.6) [a] (0.003, 32.8) [a] (0.0035, 34.1) [a] (0.004, 34.5) [a] (0.005, 35.3) [a] (0.0055, 35.4) [a] (0.006, 35.5) [a] (0.0065, 35.9) [a] (0.007, 36.4) [a] (0.0075, 36.6) [a] (0.008, 36.7) [a] (0.009, 37.1) [a] (0.0095, 37.4) [a] (0.01, 37.5) [a] (0.0105, 38.0) [a] (0.011, 38.1) [a] (0.0115, 38.3) [a] (0.012, 38.4) [a] (0.0125, 38.5) [a] (0.0135, 38.6) [a] (0.0145, 38.9) [a] (0.015, 39.2) [a] (0.016, 39.3) [a] (0.0165, 39.4) [a] (0.017, 39.5) [a] (0.0175, 39.6) [a] (0.0185, 39.7) [a] (0.019, 39.8) [a] (0.0195, 39.9) [a] (0.02, 40.0) [a] (0.0205, 40.2) [a] (0.021, 40.7) [a] (0.0215, 40.8) [a] (0.022, 41.1) [a] (0.023, 41.2) [a] (0.0245, 41.4) [a] (0.025, 41.5) [a] (0.0265, 41.6) [a] (0.027, 41.8) [a] (0.0275, 41.9) [a] (0.029, 42.2) [a] (0.0295, 42.3) [a] (0.03, 42.4) [a] (0.0305, 42.5) [a] (0.0315, 42.7) [a] (0.032, 42.8) [a] (0.0335, 42.9) [a] (0.034, 43.0) [a] (0.0345, 43.1) [a] (0.037, 43.2) [a] (0.0385, 43.3) [a] (0.0395, 43.4) [a] (0.04, 43.6) [a] (0.042, 43.7) [a] (0.0435, 43.8) [a] (0.044, 43.9) [a] (0.046, 44.0) [a] (0.047, 44.1) [a] (0.0485, 44.3) [a] (0.0495, 44.4) [a] (0.0505, 44.5) [a] (0.0515, 44.6) [a] (0.0535, 44.8) [a] (0.0545, 45.0) [a] (0.0555, 45.1) [a] (0.056, 45.2) [a] (0.0565, 45.3) [a] (0.058, 45.4) [a] (0.0585, 45.6) [a] (0.06, 45.7) [a] (0.0605, 45.8) [a] (0.061, 46.0) [a] (0.0635, 46.1) [a] (0.064, 46.2) [a] (0.065, 46.4) [a] (0.0655, 46.5) [a] (0.066, 46.6) [a] (0.0665, 46.7) [a] (0.0675, 46.8) [a] (0.0685, 46.9) [a] (0.07, 47.0) [a] (0.0705, 47.1) [a] (0.0715, 47.2) [a] (0.072, 47.3) [a] (0.0725, 47.4) [a] (0.073, 47.5) [a] (0.0735, 47.6) [a] (0.074, 47.8) [a] (0.0745, 47.9) [a] (0.0755, 48.0) [a] (0.0765, 48.1) [a] (0.077, 48.2) [a] (0.0775, 48.3) [a] (0.0785, 48.6) [a] (0.0795, 48.7) [a] (0.0815, 48.8) [a] (0.0825, 48.9) [a] (0.0835, 49.0) [a] (0.085, 49.1) [a] (0.0855, 49.2) [a] (0.087, 49.3) [a] (0.0875, 49.4) [a] (0.088, 49.5) [a] (0.0895, 49.6) [a] (0.0915, 49.7) [a] (0.092, 49.8) [a] (0.0935, 49.9) [a] (0.094, 50.1) [a] (0.095, 50.2) [a] (0.097, 50.3) [a] (0.098, 50.4) [a] (0.0995, 50.5) [a] (0.1015, 50.8) [a] (0.102, 50.9) [a] (0.1035, 51.0) [a] (0.1045, 51.1) [a] (0.105, 51.2) [a] (0.1075, 51.3) [a] (0.1085, 51.4) [a] (0.1095, 51.5) [a] (0.112, 51.6) [a] (0.113, 51.7) [a] (0.1135, 51.8) [a] (0.114, 52.2) [a] (0.1145, 52.3) [a] (0.1155, 52.4) [a] (0.116, 52.5) [a] (0.1165, 52.7) [a] (0.1175, 52.8) [a] (0.1185, 52.9) [a] (0.119, 53.0) [a] (0.1195, 53.3) [a] (0.12, 53.5) [a] (0.1205, 53.6) [a] (0.121, 53.7) [a] (0.1215, 53.8) [a] (0.1225, 54.0) [a] (0.123, 54.1) [a] (0.1235, 54.2) [a] (0.124, 54.4) [a] (0.125, 54.5) [a] (0.1255, 54.7) [a] (0.1265, 54.8) [a] (0.127, 54.9) [a] (0.1275, 55.0) [a] (0.128, 55.1) [a] (0.129, 55.4) [a] (0.1295, 55.5) [a] (0.131, 55.6) [a] (0.1325, 55.7) [a] (0.133, 55.8) [a] (0.1355, 55.9) [a] (0.1375, 56.0) [a] (0.138, 56.1) [a] (0.139, 56.3) [a] (0.14, 56.7) [a] (0.1405, 56.8) [a] (0.142, 57.0) [a] (0.1425, 57.1) [a] (0.1455, 57.2) [a] (0.146, 57.3) [a] (0.1465, 57.5) [a] (0.147, 57.7) [a] (0.1475, 57.8) [a] (0.148, 58.0) [a] (0.1485, 58.1) [a] (0.149, 58.2) [a] (0.1495, 58.3) [a] (0.15, 58.6) [a] (0.151, 58.8) [a] (0.152, 58.9) [a] (0.1525, 59.0) [a] (0.1535, 59.1) [a] (0.155, 59.3) [a] (0.1555, 59.4) [a] (0.156, 59.5) [a] (0.157, 59.7) [a] (0.1575, 60.0) [a] (0.158, 60.2) [a] (0.161, 60.3) [a] (0.1615, 60.5) [a] (0.162, 60.6) [a] (0.1625, 60.9) [a] (0.1635, 61.0) [a] (0.164, 61.1) [a] (0.1645, 61.2) [a] (0.1655, 61.3) [a] (0.166, 61.5) [a] (0.1665, 61.6) [a] (0.1675, 61.8) [a] (0.168, 62.2) [a] (0.1685, 62.4) [a] (0.169, 62.6) [a] (0.1695, 62.7) [a] (0.1705, 62.9) [a] (0.171, 63.0) [a] (0.172, 63.1) [a] (0.1725, 63.2) [a] (0.173, 63.3) [a] (0.1735, 63.4) [a] (0.174, 63.6) [a] (0.175, 63.7) [a] (0.176, 63.8) [a] (0.177, 64.0) [a] (0.178, 64.1) [a] (0.1785, 64.3) [a] (0.179, 64.4) [a] (0.18, 64.6) [a] (0.182, 64.7) [a] (0.183, 64.9) [a] (0.1845, 65.0) [a] (0.186, 65.1) [a] (0.1865, 65.2) [a] (0.187, 65.5) [a] (0.188, 65.6) [a] (0.1895, 65.8) [a] (0.1905, 65.9) [a] (0.191, 66.0) [a] (0.192, 66.1) [a] (0.193, 66.3) [a] (0.194, 66.6) [a] (0.195, 66.9) [a] (0.197, 67.0) [a] (0.1975, 67.1) [a] (0.198, 67.2) [a] (0.1985, 67.4) [a] (0.2, 67.6) [a] (0.2005, 67.8) [a] (0.201, 67.9) [a] (0.203, 68.1) [a] (0.2035, 68.4) [a] (0.204, 68.5) [a] (0.2045, 68.6) [a] (0.2055, 68.8) [a] (0.206, 68.9) [a] (0.2065, 69.0) [a] (0.207, 69.1) [a] (0.208, 69.2) [a] (0.209, 69.3) [a] (0.21, 69.4) [a] (0.212, 69.5) [a] (0.2135, 69.6) [a] (0.214, 69.7) [a] (0.215, 69.8) [a] (0.2155, 69.9) [a] (0.2165, 70.0) [a] (0.2175, 70.1) [a] (0.218, 70.5) [a] (0.2205, 70.6) [a] (0.2215, 70.8) [a] (0.222, 71.0) [a] (0.223, 71.2) [a] (0.2235, 71.4) [a] (0.225, 71.7) [a] (0.2255, 71.8) [a] (0.227, 72.2) [a] (0.2275, 72.3) [a] (0.228, 72.4) [a] (0.2285, 72.5) [a] (0.23, 72.6) [a] (0.2305, 72.7) [a] (0.2315, 73.0) [a] (0.233, 73.1) [a] (0.2335, 73.2) [a] (0.234, 73.3) [a] (0.2345, 73.4) [a] (0.235, 73.5) [a] (0.2365, 73.6) [a] (0.2375, 73.7) [a] (0.2385, 73.8) [a] (0.24, 74.0) [a] (0.2405, 74.1) [a] (0.2415, 74.2) [a] (0.2425, 74.4) [a] (0.244, 74.5) [a] (0.2445, 74.6) [a] (0.2455, 74.8) [a] (0.246, 74.9) [a] (0.2465, 75.0) [a] (0.2475, 75.2) [a] (0.2485, 75.3) [a] (0.2495, 75.5) [a] (0.25, 75.6) [a] (0.2505, 75.7) [a] (0.251, 75.8) [a] (0.2515, 75.9) [a] (0.252, 76.0) [a] (0.2525, 76.1) [a] (0.253, 76.2) [a] (0.254, 76.4) [a] (0.2555, 76.5) [a] (0.256, 76.7) [a] (0.2565, 76.9) [a] (0.258, 77.0) [a] (0.2595, 77.1) [a] (0.2605, 77.2) [a] (0.261, 77.3) [a] (0.2625, 77.4) [a] (0.263, 77.5) [a] (0.2635, 77.6) [a] (0.264, 77.9) [a] (0.2655, 78.0) [a] (0.266, 78.2) [a] (0.267, 78.3) [a] (0.2675, 78.4) [a] (0.268, 78.5) [a] (0.2685, 78.6) [a] (0.2695, 78.7) [a] (0.27, 78.8) [a] (0.271, 78.9) [a] (0.272, 79.0) [a] (0.273, 79.1) [a] (0.274, 79.2) [a] (0.2745, 79.3) [a] (0.2755, 79.4) [a] (0.277, 79.5) [a] (0.2785, 79.6) [a] (0.28, 79.7) [a] (0.2815, 79.8) [a] (0.282, 79.9) [a] (0.283, 80.3) [a] (0.2855, 80.4) [a] (0.2865, 80.5) [a] (0.287, 80.7) [a] (0.2875, 80.9) [a] (0.288, 81.0) [a] (0.289, 81.1) [a] (0.2895, 81.2) [a] (0.2905, 81.4) [a] (0.291, 81.5) [a] (0.2915, 81.6) [a] (0.2925, 81.7) [a] (0.293, 81.8) [a] (0.294, 82.0) [a] (0.2945, 82.1) [a] (0.2955, 82.3) [a] (0.296, 82.4) [a] (0.298, 82.5) [a] (0.299, 82.6) [a] (0.3005, 82.7) [a] (0.3015, 82.8) [a] (0.303, 82.9) [a] (0.305, 83.0) [a] (0.3055, 83.1) [a] (0.3065, 83.2) [a] (0.308, 83.3) [a] (0.3085, 83.5) [a] (0.309, 83.6) [a] (0.3095, 83.9) [a] (0.311, 84.0) [a] (0.312, 84.1) [a] (0.3125, 84.4) [a] (0.3145, 84.5) [a] (0.3155, 84.6) [a] (0.3165, 84.7) [a] (0.3175, 84.9) [a] (0.3185, 85.0) [a] (0.319, 85.1) [a] (0.3195, 85.2) [a] (0.32, 85.4) [a] (0.3215, 85.5) [a] (0.323, 85.6) [a] (0.3245, 85.7) [a] (0.3265, 85.8) [a] (0.3275, 85.9) [a] (0.3285, 86.0) [a] (0.331, 86.1) [a] (0.332, 86.2) [a] (0.3325, 86.3) [a] (0.3335, 86.4) [a] (0.334, 86.5) [a] (0.336, 86.6) [a] (0.337, 86.7) [a] (0.3385, 86.8) [a] (0.3395, 86.9) [a] (0.34, 87.2) [a] (0.3415, 87.3) [a] (0.342, 87.4) [a] (0.3425, 87.5) [a] (0.3435, 87.6) [a] (0.345, 87.7) [a] (0.3455, 87.8) [a] (0.346, 87.9) [a] (0.347, 88.0) [a] (0.348, 88.1) [a] (0.3485, 88.2) [a] (0.35, 88.3) [a] (0.3505, 88.4) [a] (0.3515, 88.6) [a] (0.352, 88.7) [a] (0.3525, 88.8) [a] (0.3535, 88.9) [a] (0.3545, 89.2) [a] (0.356, 89.3) [a] (0.357, 89.4) [a] (0.358, 89.5) [a] (0.359, 89.6) [a] (0.36, 89.8) [a] (0.3605, 89.9) [a] (0.361, 90.0) [a] (0.362, 90.1) [a] (0.363, 90.2) [a] (0.3635, 90.3) [a] (0.3645, 90.4) [a] (0.365, 90.5) [a] (0.3665, 90.6) [a] (0.369, 90.7) [a] (0.3695, 90.8) [a] (0.37, 90.9) [a] (0.371, 91.0) [a] (0.3715, 91.1) [a] (0.3725, 91.2) [a] (0.373, 91.3) [a] (0.374, 91.5) [a] (0.375, 91.6) [a] (0.377, 91.7) [a] (0.3785, 91.8) [a] (0.3795, 91.9) [a] (0.38, 92.0) [a] (0.381, 92.2) [a] (0.382, 92.3) [a] (0.3835, 92.4) [a] (0.384, 92.5) [a] (0.3845, 92.6) [a] (0.386, 92.7) [a] (0.3875, 92.8) [a] (0.3895, 92.9) [a] (0.3905, 93.0) [a] (0.392, 93.1) [a] (0.3935, 93.2) [a] (0.394, 93.4) [a] (0.3945, 93.5) [a] (0.395, 93.6) [a] (0.3955, 93.8) [a] (0.397, 93.9) [a] (0.3975, 94.0) [a] (0.3985, 94.1) [a] (0.4, 94.2) [a] (0.401, 94.5) [a] (0.402, 94.6) [a] (0.403, 94.7) [a] (0.404, 94.8) [a] (0.405, 94.9) [a] (0.406, 95.0) [a] (0.4065, 95.1) [a] (0.4075, 95.3) [a] (0.41, 95.4) [a] (0.4105, 95.6) [a] (0.411, 95.7) [a] (0.412, 95.8) [a] (0.4125, 96.0) [a] (0.4135, 96.3) [a] (0.4145, 96.4) [a] (0.4155, 96.5) [a] (0.4165, 96.7) [a] (0.417, 96.9) [a] (0.418, 97.0) [a] (0.4185, 97.1) [a] (0.42, 97.2) [a] (0.421, 97.3) [a] (0.4225, 97.5) [a] (0.423, 97.6) [a] (0.4245, 97.7) [a] (0.4265, 97.8) [a] (0.427, 97.9) [a] (0.4275, 98.1) [a] (0.429, 98.2) [a] (0.4295, 98.3) [a] (0.43, 98.4) [a] (0.4305, 98.5) [a] (0.431, 98.6) [a] (0.4315, 98.7) [a] (0.432, 99.0) [a] (0.4325, 99.2) [a] (0.433, 99.3) [a] (0.434, 99.4) [a] (0.435, 99.5) [a] (0.4355, 99.6) [a] (0.436, 99.7) [a] (0.438, 99.9) [a] (0.4385, 100.1) [a] (0.4395, 100.2) [a] (0.4405, 100.5) [a] (0.441, 100.9) [a] (0.442, 101.3) [a] (0.443, 101.6) [a] (0.444, 101.7) [a] (0.445, 102.0) [a] (0.4455, 102.1) [a] (0.4465, 102.2) [a] (0.4485, 102.5) [a] (0.449, 102.6) [a] (0.45, 102.7) [a] (0.4505, 102.8) [a] (0.4515, 102.9) [a] (0.4535, 103.2) [a] (0.454, 103.3) [a] (0.4555, 103.5) [a] (0.4565, 103.6) [a] (0.458, 103.7) [a] (0.4585, 103.8) [a] (0.4595, 103.9) [a] (0.4605, 104.0) [a] (0.461, 104.1) [a] (0.462, 104.2) [a] (0.4635, 104.3) [a] (0.464, 104.4) [a] (0.4645, 104.5) [a] (0.465, 104.6) [a] (0.466, 104.8) [a] (0.4665, 104.9) [a] (0.467, 105.0) [a] (0.468, 105.1) [a] (0.4685, 105.2) [a] (0.4695, 105.3) [a] (0.4705, 105.7) [a] (0.471, 105.8) [a] (0.4715, 105.9) [a] (0.473, 106.2) [a] (0.474, 106.3) [a] (0.475, 106.4) [a] (0.4765, 106.5) [a] (0.4775, 106.6) [a] (0.478, 106.7) [a] (0.479, 106.8) [a] (0.48, 107.0) [a] (0.481, 107.1) [a] (0.482, 107.2) [a] (0.483, 107.3) [a] (0.484, 107.6) [a] (0.485, 107.8) [a] (0.486, 108.0) [a] (0.4865, 108.3) [a] (0.487, 108.4) [a] (0.4875, 108.5) [a] (0.4895, 108.8) [a] (0.4915, 109.0) [a] (0.492, 109.2) [a] (0.493, 109.5) [a] (0.4935, 109.6) [a] (0.494, 109.7) [a] (0.4945, 109.8) [a] (0.4955, 109.9) [a] (0.496, 110.0) [a] (0.4965, 110.1) [a] (0.497, 110.2) [a] (0.5, 110.3) [a] (0.5005, 110.5) [a] (0.501, 110.6) [a] (0.5015, 110.8) [a] (0.502, 111.0) [a] (0.5025, 111.1) [a] (0.503, 111.3) [a] (0.5035, 111.4) [a] (0.5045, 111.5) [a] (0.505, 111.6) [a] (0.5055, 111.7) [a] (0.5065, 111.8) [a] (0.507, 111.9) [a] (0.509, 112.0) [a] (0.5095, 112.1) [a] (0.51, 112.2) [a] (0.511, 112.3) [a] (0.5115, 112.5) [a] (0.512, 112.6) [a] (0.5125, 112.7) [a] (0.5135, 112.8) [a] (0.5145, 112.9) [a] (0.5155, 113.1) [a] (0.516, 113.2) [a] (0.5175, 113.5) [a] (0.5195, 113.6) [a] (0.52, 113.7) [a] (0.5205, 113.8) [a] (0.5215, 113.9) [a] (0.523, 114.0) [a] (0.5235, 114.1) [a] (0.524, 114.3) [a] (0.5245, 114.5) [a] (0.525, 114.6) [a] (0.5255, 114.7) [a] (0.526, 114.8) [a] (0.527, 114.9) [a] (0.5275, 115.1) [a] (0.528, 115.2) [a] (0.529, 115.4) [a] (0.53, 115.5) [a] (0.5305, 115.6) [a] (0.5325, 115.8) [a] (0.534, 116.1) [a] (0.5345, 116.2) [a] (0.5365, 116.4) [a] (0.5375, 116.5) [a] (0.5385, 116.6) [a] (0.539, 116.7) [a] (0.54, 116.9) [a] (0.541, 117.0) [a] (0.5415, 117.1) [a] (0.542, 117.4) [a] (0.544, 117.5) [a] (0.545, 117.6) [a] (0.546, 117.7) [a] (0.5465, 117.8) [a] (0.5485, 117.9) [a] (0.5495, 118.0) [a] (0.55, 118.1) [a] (0.551, 118.2) [a] (0.552, 118.3) [a] (0.5525, 118.4) [a] (0.554, 118.5) [a] (0.5545, 118.6) [a] (0.555, 118.8) [a] (0.5555, 119.0) [a] (0.556, 119.1) [a] (0.5575, 119.2) [a] (0.558, 119.4) [a] (0.5585, 119.5) [a] (0.56, 119.6) [a] (0.5615, 119.7) [a] (0.562, 119.8) [a] (0.563, 120.0) [a] (0.5635, 120.1) [a] (0.5655, 120.3) [a] (0.566, 120.4) [a] (0.5665, 120.5) [a] (0.5675, 120.6) [a] (0.568, 120.7) [a] (0.569, 120.8) [a] (0.5705, 120.9) [a] (0.5715, 121.0) [a] (0.573, 121.1) [a] (0.575, 121.2) [a] (0.5755, 121.3) [a] (0.577, 121.4) [a] (0.5775, 121.5) [a] (0.578, 121.6) [a] (0.579, 121.7) [a] (0.5795, 121.8) [a] (0.5805, 122.0) [a] (0.582, 122.1) [a] (0.5835, 122.2) [a] (0.5845, 122.3) [a] (0.5855, 122.4) [a] (0.586, 122.5) [a] (0.587, 122.6) [a] (0.5875, 122.7) [a] (0.5885, 122.8) [a] (0.589, 123.0) [a] (0.5895, 123.1) [a] (0.59, 123.2) [a] (0.5905, 123.3) [a] (0.592, 123.4) [a] (0.593, 123.5) [a] (0.594, 123.6) [a] (0.595, 123.7) [a] (0.5955, 123.8) [a] (0.596, 123.9) [a] (0.5965, 124.0) [a] (0.5975, 124.3) [a] (0.5985, 124.4) [a] (0.6, 124.5) [a] (0.601, 124.6) [a] (0.602, 124.7) [a] (0.6025, 124.8) [a] (0.603, 124.9) [a] (0.6045, 125.0) [a] (0.605, 125.1) [a] (0.606, 125.2) [a] (0.609, 125.3) [a] (0.6095, 125.5) [a] (0.6115, 125.6) [a] (0.613, 125.7) [a] (0.6135, 125.8) [a] (0.6145, 125.9) [a] (0.616, 126.0) [a] (0.6175, 126.2) [a] (0.6195, 126.3) [a] (0.6205, 126.4) [a] (0.621, 126.5) [a] (0.622, 126.6) [a] (0.623, 126.7) [a] (0.6245, 126.8) [a] (0.626, 126.9) [a] (0.6265, 127.0) [a] (0.627, 127.1) [a] (0.6275, 127.2) [a] (0.6285, 127.3) [a] (0.63, 127.4) [a] (0.632, 127.5) [a] (0.6325, 127.6) [a] (0.6335, 127.7) [a] (0.6345, 127.8) [a] (0.6355, 127.9) [a] (0.636, 128.0) [a] (0.637, 128.1) [a] (0.638, 128.2) [a] (0.639, 128.3) [a] (0.6395, 128.4) [a] (0.64, 128.7) [a] (0.6405, 128.8) [a] (0.6415, 128.9) [a] (0.642, 129.0) [a] (0.6425, 129.1) [a] (0.643, 129.2) [a] (0.644, 129.3) [a] (0.6445, 129.4) [a] (0.646, 129.5) [a] (0.6465, 129.6) [a] (0.6475, 129.8) [a] (0.649, 129.9) [a] (0.65, 130.0) [a] (0.651, 130.1) [a] (0.6525, 130.3) [a] (0.6535, 130.4) [a] (0.654, 130.5) [a] (0.655, 130.7) [a] (0.6565, 130.9) [a] (0.657, 131.1) [a] (0.6585, 131.2) [a] (0.6595, 131.3) [a] (0.6605, 131.5) [a] (0.661, 131.6) [a] (0.6615, 131.7) [a] (0.6625, 131.8) [a] (0.664, 131.9) [a] (0.665, 132.1) [a] (0.6655, 132.2) [a] (0.666, 132.3) [a] (0.667, 132.4) [a] (0.668, 132.5) [a] (0.6695, 132.6) [a] (0.67, 132.7) [a] (0.671, 132.9) [a] (0.6715, 133.0) [a] (0.673, 133.2) [a] (0.6735, 133.4) [a] (0.674, 133.5) [a] (0.6745, 133.6) [a] (0.6755, 134.0) [a] (0.676, 134.1) [a] (0.678, 134.2) [a] (0.6785, 134.3) [a] (0.679, 134.6) [a] (0.68, 134.7) [a] (0.681, 134.8) [a] (0.6815, 134.9) [a] (0.6825, 135.0) [a] (0.683, 135.1) [a] (0.684, 135.2) [a] (0.6845, 135.3) [a] (0.6855, 135.4) [a] (0.686, 135.6) [a] (0.6865, 135.9) [a] (0.687, 136.0) [a] (0.6875, 136.3) [a] (0.688, 136.5) [a] (0.69, 136.6) [a] (0.6915, 136.7) [a] (0.693, 136.8) [a] (0.694, 136.9) [a] (0.6955, 137.0) [a] (0.697, 137.1) [a] (0.6975, 137.2) [a] (0.698, 137.4) [a] (0.6985, 137.6) [a] (0.6995, 137.7) [a] (0.7, 137.9) [a] (0.701, 138.0) [a] (0.703, 138.1) [a] (0.7035, 138.2) [a] (0.704, 138.3) [a] (0.7045, 138.4) [a] (0.705, 138.7) [a] (0.7055, 138.8) [a] (0.706, 138.9) [a] (0.7065, 139.2) [a] (0.707, 139.3) [a] (0.7075, 139.4) [a] (0.7085, 139.5) [a] (0.71, 139.6) [a] (0.7105, 140.0) [a] (0.711, 140.1) [a] (0.712, 140.2) [a] (0.713, 140.3) [a] (0.7145, 140.4) [a] (0.715, 140.6) [a] (0.7155, 140.7) [a] (0.716, 140.8) [a] (0.717, 140.9) [a] (0.7175, 141.0) [a] (0.718, 141.1) [a] (0.719, 141.3) [a] (0.7195, 141.4) [a] (0.72, 141.6) [a] (0.7205, 141.8) [a] (0.7215, 141.9) [a] (0.722, 142.2) [a] (0.723, 142.3) [a] (0.724, 142.5) [a] (0.7245, 142.6) [a] (0.725, 142.7) [a] (0.726, 143.4) [a] (0.7265, 143.7) [a] (0.727, 144.1) [a] (0.7275, 144.2) [a] (0.728, 144.4) [a] (0.7285, 144.5) [a] (0.729, 144.7) [a] (0.7295, 144.8) [a] (0.73, 144.9) [a] (0.7305, 145.0) [a] (0.731, 145.1) [a] (0.7325, 145.4) [a] (0.733, 145.6) [a] (0.7345, 145.8) [a] (0.735, 146.0) [a] (0.7355, 146.2) [a] (0.7365, 146.3) [a] (0.737, 146.5) [a] (0.7375, 146.6) [a] (0.738, 146.7) [a] (0.7385, 146.8) [a] (0.7395, 146.9) [a] (0.74, 147.1) [a] (0.7405, 147.3) [a] (0.741, 147.4) [a] (0.7415, 147.5) [a] (0.742, 147.7) [a] (0.7425, 147.9) [a] (0.743, 148.3) [a] (0.7435, 148.5) [a] (0.7445, 148.9) [a] (0.745, 149.2) [a] (0.746, 149.6) [a] (0.7465, 150.2) [a] (0.747, 150.4) [a] (0.7475, 150.7) [a] (0.7485, 151.0) [a] (0.749, 151.1) [a] (0.7495, 151.2) [a] (0.75, 151.4) [a] (0.751, 151.5) [a] (0.7515, 151.6) [a] (0.7525, 151.7) [a] (0.753, 151.9) [a] (0.7535, 152.0) [a] (0.754, 152.1) [a] (0.755, 152.4) [a] (0.7555, 152.5) [a] (0.756, 152.9) [a] (0.7565, 153.4) [a] (0.757, 153.7) [a] (0.7575, 153.8) [a] (0.758, 154.1) [a] (0.7585, 154.3) [a] (0.759, 154.4) [a] (0.7595, 154.5) [a] (0.76, 155.0) [a] (0.7605, 155.3) [a] (0.761, 155.5) [a] (0.7615, 155.6) [a] (0.762, 155.9) [a] (0.7625, 156.0) [a] (0.763, 156.3) [a] (0.764, 156.9) [a] (0.7645, 157.2) [a] (0.766, 157.6) [a] (0.7665, 157.9) [a] (0.767, 158.0) [a] (0.7675, 158.2) [a] (0.768, 158.4) [a] (0.7685, 158.5) [a] (0.769, 158.6) [a] (0.7695, 159.3) [a] (0.77, 159.5) [a] (0.7705, 159.6) [a] (0.771, 159.8) [a] (0.7715, 160.0) [a] (0.7725, 160.2) [a] (0.773, 160.4) [a] (0.7735, 161.0) [a] (0.7745, 161.2) [a] (0.775, 161.6) [a] (0.7755, 161.8) [a] (0.776, 162.1) [a] (0.7765, 162.2) [a] (0.777, 162.5) [a] (0.7775, 162.8) [a] (0.778, 163.6) [a] (0.7795, 163.7) [a] (0.78, 164.0) [a] (0.7805, 164.6) [a] (0.781, 165.0) [a] (0.7815, 166.3) [a] (0.782, 166.5) [a] (0.7825, 166.6) [a] (0.783, 167.1) [a] (0.7835, 167.2) [a] (0.784, 168.0) [a] (0.7845, 168.2) [a] (0.785, 168.4) [a] (0.7855, 168.5) [a] (0.786, 168.7) [a] (0.7865, 169.4) [a] (0.787, 169.5) [a] (0.7875, 170.3) [a] (0.788, 171.7) [a] (0.7885, 171.8) [a] (0.789, 172.0) [a] (0.79, 172.2) [a] (0.7905, 172.5) [a] (0.791, 172.9) [a] (0.7915, 173.0) [a] (0.792, 173.9) [a] (0.793, 174.3) [a] (0.7935, 174.5) [a] (0.7945, 175.0) [a] (0.795, 175.3) [a] (0.7955, 176.7) [a] (0.796, 178.9) [a] (0.7965, 179.5) [a] (0.797, 180.7) [a] (0.7975, 180.8) [a] (0.798, 180.9) [a] (0.7985, 181.5) [a] (0.799, 181.8) [a] (0.7995, 182.3) [a] (0.8, 182.6) [a] (0.8005, 183.5) [a] (0.801, 184.3) [a] (0.8015, 184.8) [a] (0.802, 184.9) [a] (0.8025, 185.2) [a] (0.8035, 186.6) [a] (0.804, 186.7) [a] (0.8045, 187.1) [a] (0.805, 187.5) [a] (0.8055, 187.7) [a] (0.806, 188.3) [a] (0.8065, 188.4) [a] (0.807, 188.6) [a] (0.8075, 189.2) [a] (0.808, 189.4) [a] (0.8085, 190.3) [a] (0.809, 190.7) [a] (0.81, 191.0) [a] (0.8105, 191.2) [a] (0.811, 192.0) [a] (0.8115, 192.1) [a] (0.8125, 192.5) [a] (0.813, 192.7) [a] (0.8135, 192.8) [a] (0.814, 193.0) [a] (0.8145, 193.3) [a] (0.815, 193.4) [a] (0.8155, 194.1) [a] (0.816, 194.3) [a] (0.8165, 195.1) [a] (0.818, 195.2) [a] (0.8185, 195.3) [a] (0.819, 195.4) [a] (0.8195, 196.0) [a] (0.82, 196.8) [a] (0.8205, 197.2) [a] (0.821, 197.6) [a] (0.8215, 198.0) [a] (0.822, 198.4) [a] (0.8225, 198.5) [a] (0.8235, 198.7) [a] (0.824, 198.9) [a] (0.8245, 199.1) [a] (0.825, 199.7) [a] (0.8255, 200.3) [a] (0.826, 200.7) [a] (0.827, 200.9) [a] (0.8275, 201.4) [a] (0.828, 201.5) [a] (0.8285, 202.4) [a] (0.829, 202.6) [a] (0.8295, 202.8) [a] (0.83, 203.6) [a] (0.8305, 204.3) [a] (0.831, 204.7) [a] (0.832, 204.8) [a] (0.8325, 205.0) [a] (0.833, 205.7) [a] (0.8335, 206.0) [a] (0.834, 206.1) [a] (0.8345, 206.3) [a] (0.835, 206.9) [a] (0.8365, 207.6) [a] (0.837, 207.8) [a] (0.838, 209.3) [a] (0.8385, 209.8) [a] (0.839, 209.9) [a] (0.8395, 210.3) [a] (0.84, 210.8) [a] (0.8405, 211.3) [a] (0.841, 211.6) [a] (0.8415, 211.8) [a] (0.842, 211.9) [a] (0.8425, 212.0) [a] (0.8435, 212.4) [a] (0.8445, 212.6) [a] (0.845, 213.2) [a] (0.8455, 213.3) [a] (0.846, 213.8) [a] (0.8465, 214.0) [a] (0.847, 214.1) [a] (0.8475, 214.3) [a] (0.848, 214.4) [a] (0.8485, 214.9) [a] (0.849, 215.5) [a] (0.8495, 216.8) [a] (0.85, 218.3) [a] (0.8505, 218.4) [a] (0.851, 219.1) [a] (0.8515, 219.6) [a] (0.852, 220.2) [a] (0.8525, 220.4) [a] (0.853, 220.5) [a] (0.854, 220.6) [a] (0.8545, 220.8) [a] (0.855, 221.0) [a] (0.8555, 221.4) [a] (0.856, 221.7) [a] (0.8565, 222.1) [a] (0.857, 222.4) [a] (0.8575, 223.0) [a] (0.858, 223.1) [a] (0.8585, 223.2) [a] (0.859, 223.3) [a] (0.8595, 223.7) [a] (0.86, 224.1) [a] (0.8605, 224.9) [a] (0.861, 225.1) [a] (0.8615, 225.6) [a] (0.862, 225.7) [a] (0.863, 226.0) [a] (0.8635, 226.1) [a] (0.864, 226.7) [a] (0.8645, 226.8) [a] (0.865, 227.1) [a] (0.8655, 227.2) [a] (0.866, 227.6) [a] (0.8665, 227.7) [a] (0.867, 228.0) [a] (0.8675, 228.1) [a] (0.868, 228.5) [a] (0.8685, 228.6) [a] (0.869, 229.3) [a] (0.8695, 229.7) [a] (0.87, 230.2) [a] (0.8705, 230.4) [a] (0.871, 231.0) [a] (0.8715, 231.9) [a] (0.872, 232.2) [a] (0.8725, 233.0) [a] (0.873, 234.0) [a] (0.874, 235.8) [a] (0.875, 235.9) [a] (0.876, 236.4) [a] (0.8765, 236.6) [a] (0.877, 236.8) [a] (0.8775, 237.6) [a] (0.8785, 238.3) [a] (0.879, 238.4) [a] (0.8795, 238.8) [a] (0.88, 238.9) [a] (0.8805, 239.0) [a] (0.881, 239.5) [a] (0.8815, 239.6) [a] (0.882, 239.8) [a] (0.8825, 240.4) [a] (0.883, 240.6) [a] (0.8835, 240.8) [a] (0.884, 241.3) [a] (0.8845, 241.6) [a] (0.885, 242.8) [a] (0.8855, 243.0) [a] (0.886, 243.4) [a] (0.8865, 243.6) [a] (0.887, 244.5) [a] (0.8875, 244.7) [a] (0.888, 245.1) [a] (0.889, 245.5) [a] (0.89, 246.1) [a] (0.8905, 247.8) [a] (0.891, 248.4) [a] (0.8915, 249.0) [a] (0.892, 250.0) [a] (0.8925, 252.1) [a] (0.893, 252.3) [a] (0.8935, 252.4) [a] (0.894, 252.9) [a] (0.8945, 253.5) [a] (0.895, 254.0) [a] (0.8955, 254.3) [a] (0.896, 254.5) [a] (0.8965, 254.7) [a] (0.897, 254.9) [a] (0.8975, 256.2) [a] (0.898, 256.3) [a] (0.8985, 257.2) [a] (0.899, 259.6) [a] (0.8995, 259.8) [a] (0.9, 260.1) [a] (0.9005, 260.5) [a] (0.901, 260.8) [a] (0.9015, 261.9) [a] (0.902, 262.6) [a] (0.9025, 263.5) [a] (0.903, 264.7) [a] (0.9035, 264.8) [a] (0.904, 266.1) [a] (0.9045, 266.3) [a] (0.905, 268.0) [a] (0.9055, 268.5) [a] (0.906, 268.7) [a] (0.9065, 269.1) [a] (0.907, 269.4) [a] (0.9075, 269.7) [a] (0.908, 270.6) [a] (0.9085, 270.8) [a] (0.9095, 271.0) [a] (0.91, 271.2) [a] (0.9105, 271.3) [a] (0.911, 272.1) [a] (0.9115, 273.2) [a] (0.912, 273.3) [a] (0.9125, 274.2) [a] (0.913, 275.7) [a] (0.9135, 276.3) [a] (0.914, 276.8) [a] (0.9145, 277.2) [a] (0.915, 277.4) [a] (0.9155, 278.2) [a] (0.916, 278.7) [a] (0.9165, 278.9) [a] (0.9175, 279.9) [a] (0.9185, 280.1) [a] (0.919, 280.4) [a] (0.9195, 281.7) [a] (0.92, 282.9) [a] (0.9205, 283.8) [a] (0.921, 284.4) [a] (0.9215, 284.6) [a] (0.922, 285.9) [a] (0.9225, 286.7) [a] (0.923, 286.8) [a] (0.9235, 286.9) [a] (0.924, 287.9) [a] (0.9245, 288.5) [a] (0.9255, 289.3) [a] (0.926, 289.6) [a] (0.9265, 290.0) [a] (0.927, 290.2) [a] (0.9275, 290.4) [a] (0.928, 290.8) [a] (0.9285, 291.0) [a] (0.929, 292.8) [a] (0.9295, 293.7) [a] (0.93, 293.8) [a] (0.9305, 294.8) [a] (0.931, 295.1) [a] (0.932, 295.2) [a] (0.9325, 295.7) [a] (0.933, 295.9) [a] (0.9335, 296.5) [a] (0.934, 296.8) [a] (0.9345, 297.4) [a] (0.935, 299.0) [a] (0.9355, 300.2) [a] (0.937, 300.5) [a] (0.9375, 300.7) [a] (0.938, 301.1) [a] (0.9385, 301.5) [a] (0.939, 301.8) [a] (0.9395, 302.3) [a] (0.94, 302.7) [a] (0.9405, 304.8) [a] (0.941, 304.9) [a] (0.9415, 305.1) [a] (0.942, 305.2) [a] (0.9425, 305.6) [a] (0.9435, 306.5) [a] (0.944, 306.8) [a] (0.9445, 307.2) [a] (0.945, 308.0) [a] (0.9455, 308.4) [a] (0.946, 308.6) [a] (0.9465, 310.7) [a] (0.947, 312.0) [a] (0.948, 312.4) [a] (0.9485, 313.4) [a] (0.949, 314.4) [a] (0.9495, 315.2) [a] (0.95, 315.4) [a] (0.951, 316.1) [a] (0.9515, 318.3) [a] (0.9525, 319.2) [a] (0.953, 319.3) [a] (0.9535, 319.5) [a] (0.954, 321.8) [a] (0.9545, 322.0) [a] (0.955, 322.7) [a] (0.9555, 323.7) [a] (0.956, 324.0) [a] (0.957, 324.7) [a] (0.9575, 325.0) [a] (0.958, 326.5) [a] (0.9585, 327.2) [a] (0.959, 328.0) [a] (0.9595, 328.3) [a] (0.96, 329.1) [a] (0.9605, 329.3) [a] (0.9615, 329.6) [a] (0.962, 330.4) [a] (0.9625, 331.0) [a] (0.963, 331.5) [a] (0.9635, 331.7) [a] (0.964, 332.3) [a] (0.9645, 333.1) [a] (0.965, 333.2) [a] (0.9655, 334.9) [a] (0.966, 335.8) [a] (0.9665, 335.9) [a] (0.967, 339.0) [a] (0.9675, 341.0) [a] (0.968, 341.8) [a] (0.9685, 342.5) [a] (0.969, 342.8) [a] (0.9695, 343.7) [a] (0.97, 345.0) [a] (0.9705, 346.2) [a] (0.971, 347.2) [a] (0.9715, 351.4) [a] (0.972, 352.0) [a] (0.9725, 353.6) [a] (0.973, 354.1) [a] (0.9735, 355.6) [a] (0.974, 355.7) [a] (0.9745, 358.1) [a] (0.975, 359.0) [a] (0.9755, 360.8) [a] (0.976, 361.8) [a] (0.9765, 363.3) [a] (0.977, 363.9) [a] (0.9775, 364.6) [a] (0.978, 370.5) [a] (0.9785, 371.8) [a] (0.979, 372.9) [a] (0.9795, 376.9) [a] (0.98, 377.4) [a] (0.9805, 389.2) [a] (0.981, 389.3) [a] (0.9815, 390.1) [a] (0.982, 392.2) [a] (0.9825, 394.7) [a] (0.983, 395.1) [a] (0.9835, 399.8) [a] (0.984, 400.7) [a] (0.9845, 403.1) [a] (0.985, 403.3) [a] (0.9855, 404.0) [a] (0.986, 407.7) [a] (0.9865, 418.1) [a] (0.987, 421.4) [a] (0.9875, 450.9) [a] (0.988, 452.4) [a] (0.9885, 461.8) [a] (0.989, 466.6) [a] (0.9895, 467.6) [a] (0.99, 480.7) [a] (0.9905, 484.9) [a] (0.991, 525.7) [a] (0.9915, 526.1) [a] (0.992, 564.4) [a] (0.9925, 569.3) [a] (0.993, 605.1) [a] (0.9935, 615.7) [a] (0.994, 631.1) [a] (0.9945, 635.6) [a] (0.995, 654.8) [a] (0.9955, 687.8) [a] (0.996, 694.5) [a] (0.9965, 701.9) [a] (0.997, 850.6) [a] (0.9975, 867.2) [a] (0.998, 875.4) [a] },{(0.0, 0.0) [b] },{(0.0, 0.0) [c] }}}

